A Review of Computer Vision Methods in Network Security

Network security has become an area of significant importance more than ever as highlighted by the eye-opening numbers of data breaches, attacks on critical infrastructure, and malware/ransomware/cryptojacker attacks that are reported almost every day. Increasingly, we are relying on networked infrastructure and with the advent of IoT, billions of devices will be connected to the internet, providing attackers with more opportunities to exploit. Traditional machine learning methods have been frequently used in the context of network security. However, such methods are more based on statistical features extracted from sources such as binaries, emails, and packet flows. On the other hand, recent years witnessed a phenomenal growth in computer vision mainly driven by the advances in the area of convolutional neural networks. At a glance, it is not trivial to see how computer vision methods are related to network security. Nonetheless, there is a significant amount of work that highlighted how methods from computer vision can be applied in network security for detecting attacks or building security solutions. In this paper, we provide a comprehensive survey of such work under three topics; i) phishing attempt detection, ii) malware detection, and iii) traffic anomaly detection. Next, we review a set of such commercial products for which public information is available and explore how computer vision methods are effectively used in those products. Finally, we discuss existing research gaps and future research directions, especially focusing on how network security research community and the industry can leverage the exponential growth of computer vision methods to build much secure networked systems.

==> extra.tex <==
\begin{table*}
%\centering
\caption{Malware Detection Approaches} \vspace{-3mm}
\begin{tabular}{p{1cm}|p{1.8cm}|p{3cm}|p{3cm}|p{1.6cm}|p{2cm}|p{2.6cm}}
%|p{0.5cm}|p{2.1cm}|p{3.4cm}|p{3cm}|p{1.6cm}|p{2cm}|p{2.6cm}|

 \hline
    \textbf{Ref}	& \textbf{Methods Used }	& \textbf{Advantages} &	\textbf{Disadvantages/ Limitations}	& \textbf{Dataset (Samples/ Families)} & \textbf{Comparison Vector}& \textbf{Performance Metrics	}\\ \hline
    \hline
    
   \cite{chapman2018sad} &	Average Hash, FLANN and random tree	& Fast method as it uses average hash and FLANN	& Accuracy is highly depending on algorithm threshold value & 	200,000/ 200	& $32 \times 32 $ image	& Recall- 83\% \newline Precision- 85\% \\ \hline 

%\cite{MD:Zhou2017} &	GIST and extreme random tree classification &	Cross validation further improves the performance of the model	& Required time and memory	& 15781/-	& 512 GIST descriptors &	Accuracy- 96.2\%\newline Recall- 97.5\%\newline Precision - 94.2\% \\ \hline

\cite{MD:Nataraj2011} &	 GIST and K-NN &	GIST feature extraction is faster than the b-gram	& This method considered only global features	& \textbf{DS1}- 1731/8 \newline \textbf{DS2}- 9458/25	& 320 GIST descriptors	& \textbf{DS1:} \newline Accuracy- 99.9\%\newline \textbf{DS2:} \newline Accuracy- 97.2\% \\ \hline

%\cite{MD:Yajamanam2018}	& GIST and k-NN	& Required only 60 GIST features	& Less efficient with large number of samples	& 9000-9312	& 60 GIST descriptors	& Accuracy - 93\% \\ \hline

\cite{MD:Han2015} & Bitmap images and entropy graphs	 & Less computation overhead and time compared to GIST methods	& Not suitable when malware binary files are packed	& 1000/50	 & N/A	& Accuracy- 97.9\% \\ \hline

\cite{MD:Han2014}	& SimHash and angular-based distance measurement algorithm &	Has reduced the computation overhead by comparing images with major blocks and has considered RGB-color  &	  The method can improve by using a parallelization technique and real time processing	& \textbf{Static}- 290 /16 \newline \textbf{Dynamic}- 560/14	& $256\times 256$ image &	  \textbf{Static:}\newline Accuracy- 98.9\% \newline \textbf{Dynamic:}\newline Accuracy- 97.3\% \\ \hline

%\cite{MD:Liu2016}	& Local mean and ensemble learning	& K-means and bagging methods used to avoid conflicts between classifiers	& Time required to train the malware classifier model&	20000/20	& $512\times 512$ image	 & Accuracy- 98.2\% \\ \hline

%\cite{MD:Choi2017}	& CNN	& Has used three convolution layers to make the model robust	& Ran out of memory when using 256x256 images 	& 2000/-	& $32 \times 32$ input image to CNN with 3 layer&	Accuracy- 96\% \\ \hline

\cite{MD:Kabanga2018}	& CNN and cross entropy	& High accuracy &	Small change in an image will lead to a misclassification	& 9458/25	 & $128 \time128$ input image to CNN with 3 layers &	Accuracy- 98\% \\ \hline

\cite{MD:Yue2017	} & CNN and weighted softmax loss	& Addressed the performance degration due to imbalance of malware family	& Need to choose the weighted values	properly & 9342/25	 & vgg-verydeep-19 CNN model with 60 layers &	Accuracy-98.63\% \\ \hline

\cite{MD:Wang2017} & CNN  and softmax function & The method is protocol independent and can detect malware in early stage & Haven't done parameter tuning, ignored temporal features and cannot  identify unknown malware traffic & 406633/- & $28 \time28$ input image to CNN with 3 layers & Accuracy-99.41\%  \\ \hline

\end{tabular}
\end{table*}

\cite{MD:Nataraj2011} &	 & 320 GIST descriptors	& \textbf{DS1}- 1731/8 \newline \textbf{DS2}- 9458/25	& & \textbf{DS1:} \newline Accuracy- 99.9\%\newline \textbf{DS2:} \newline Accuracy- 97.2\% \\ \hline

\cite{MD:Han2015} & & N/A  & 1000/50	&  & Accuracy- 97.9\% \\ \hline

\cite{MD:Han2014}	& & $256\times 256$ image	& \textbf{Static}- 290 /16 \newline \textbf{Dynamic}- 560/14	&  & \textbf{Static:}\newline Accuracy- 98.9\% \newline \textbf{Dynamic:}\newline Accuracy- 97.3\% \\ \hline

\cite{MD:Kabanga2018} & &	$128 \time128$ input image to CNN with 3 layers & 9458/25	 & 	& Accuracy- 98\% \\ \hline

\cite{MD:Yue2017	} & & vgg-verydeep-19 CNN model with 60 layers & 9342/25	  &	& Accuracy-98.63\% \\ \hline

\cite{MD:Wang2017} & & $28 \time28$ input image to CNN with 3 layers & 406633/- & & Accuracy-99.41\%  \\ \hline

using the coordinate-defining and the RGB color-defining module.  The coordinate-defining module defines the (x,y) coordinates on image matrices for binary information of each code block. Here, SimHash, a local sensitive hashing is applied to map similar binary information to same coordinates. The RGB color-defining module defines the color values of images on an image matrix. 

\begin{table*}
\scriptsize
%\centering
\caption{Malware Detection Approaches} \vspace{-3mm}
\begin{tabular}{p{0.5cm}|p{2cm}| p{2cm}|p{2cm}|p{6cm}|p{2.6cm}}
%|p{0.5cm}|p{2.1cm}|p{3.4cm}|p{3cm}|p{1.6cm}|p{2cm}|p{2.6cm}|

 \hline
\textbf{Ref}	& \textbf{Techniques Applied}	& \textbf{Image Structure} & \textbf{Dataset/Family} & \textbf{Description} & \textbf{Performance Metrics	}\\ \hline

\hline
\multicolumn{5}{c}{\textbf{Image Representation Approaches}} \\ \hline
\hline

\cite{trinius2009visual} & Treemaps, ThreadGraphs, and CWSandbox & Generic image size because of Sandbox & 2000/13 & proposed an abstraction method to make malware reports easily understandable and to enable the extraction of unique features for malware detection. & Not Given \\
\hline

\cite{han2013malware} & SimHssh, vector angular-based distance measure & 256*256 pixels of image matrices &  Not mentioned & 3 malware families (Boxed, Klez, and Evol) & Similarity (across same family) - 0.95 \newline Similarity (across diff. family) - 0.32 \\
\hline

\cite{chapman2018sad} & File Structure Decomposition &	JPEG and PNG files of variable length & 270k JPEG and 33k PNG files	& Cerber, DuQu, Hammertoss, Microcin, SyncCrypt, Tropic Trooper, ZeusVM, Zberp, APP0 Byte Stuffing, APP1: Comment Injection, Brazilian EK, CryLocker, DNSChanger, aaAa Injection, pHYs Byte Stuffing& TPR - 99.24\%, 99.31\% \newline TNR- 99.32\%, 98.88\% \\ \hline
 
\cite{han2015malware} & Bitmap Image Convertor, Entropy Graph Generator and Similarity Calculation Algorithm  & pixels of file size &  1,000 samples & 50 malware families as mentioned in the paper & Accuracy (ROC) - 97.9\%\\  
\hline



\cite{MD:Han2014}	& SimHash and angular based distance measurement & $256\times 256$ image	& \textbf{Static}- 290 /16 \newline \textbf{Dynamic}- 560/14	& \textbf{Static}- 290 samples/ 16 families \newline \textbf{Dynamic}- 560 samples/14 families & \textbf{Static:}\newline Accuracy- 98.9\% \newline \textbf{Dynamic:}\newline Accuracy- 97.3\% \\ 
\hline



\cite{shaid2014malware} & Color Mapping, API monitoring utility, Similarity measure & 64 x 4 pixel & 1101 samples & 12 malware families & Accuracy - 95-02\% to 98.92\% \\
\hline 

\hline
\multicolumn{5}{c}{\textbf{Feature Representation Approaches}} \\ \hline
\hline

\cite{kancherla2013image} & SVM, Gabor Filter, Wavelet Transformation &2-dimensional vector of fixed length of file size & 37000 samples & Virus, Trojans, Worms, Adware, Toolkits, Spyware & Accuracy (ROC) - 95.95\%\\  
\hline

\cite{MD:Nataraj2011} &	k-nearest neighbors with Euclidean distance & 320 GIST descriptors	& 9458/25	& 25 malware families &  Accuracy- 98\% \\ \hline

%\cite{nataraj2011comparative} & k-nearest neighbors with Euclidean distance, API hooking, Forensics Dumping & 
    
\cite{xiaolin2018research} & B2M, Imporved SIFT, Guassian Pyramid	& 66 byte feature descriptor & 1789 samples	& Backdoor.Win32.Agent/Bifrose/Ceckno, VirusShare, Trojan-Banker.Win32.Banbra, Trojan-Clicker.Win32.Agent, Trojan-Downloaded.Win32.Adload, Trojan-Dropper.Win32.Agent, Trojan-GameTheif.Win32.Magania, Trojan-PSW.Win32.Agent, Trojan-SPY.Win32.Agent & Accuracy (Max) - 90.32\% \newline Accuracy (Min)- 92.0\% \\ 
\hline
  
\cite{ahmadi2016novel} & forward setpwise selection algorithm, XGBoost & hex byte as a gray-scale pixel & 21741 samples & Ramnit, Lollipop,  Kelihos-ver3, Vundo, Simda, Tracur, Kelihos-ver1, Obfuscator.ACY, Gatak & Accuracy (with Img. Feat.) - 95.5\% \newline Accuracy (comb. of other feat.)- 99.40\% \\ 
\hline

\cite{xiaofang2014malware} & locality-sensitive hashing (LSH), SURF, B2M & 64*64 image vector & 8,410 samples &25 malware families & Precsion/Recall/F-Score - 80-90\% \\
\hline
 
\hline 
\multicolumn{5}{c}{\textbf{Neural Network Approaches}} \\ \hline
\hline

\cite{zhang2016irmd} & Opcode Sequence, Histogram, Dilution, Erosion, CNN & 2-Dimensional opcode images & 17808 samples & Backdoor, Net-Worm, P2P-Worm, IRC-Worm, IM-Worm, Email-Worm, Worm, Trojan Dropper, Trojan-GameThief, Trojan Banker & Accuracy (Max.) - 96.7\% \newline TPR (Max.) - 94.3\% \newline TNR (Max.) - 99.1\%  \\ 
\hline

\cite{kim2018zero} & DAE, GANS & 63*135 pixel image & 10,800 samples & Ramnit, Lollipop, Kelihos-ver3, Vundo, Simda, Tracur, Kelihos-ver1, Obfuscator.ACY, Ghatak & Accuracy (Avg.) - 96.74\%  \\ 
\hline

\cite{kim2017malware} & GANS, t-SNE Algorithm & Average of all the rows and columns of the data &  9970 samples & Ramnit, Lollipop, Kelihos-ver3, Vundo, Simda, Tracur, Kelihos-ver1, Obfuscator.ACY, Gatak & Accuracy (Avg.) - 96.39\% \\
\hline

\cite{kim2018detecting} & GANS, VAE & image size 256*128 \newline Latent Space Size - 270 dimension & 10867 samples & Ramnit, Vundo, K1, Lollipop, Simda, O.ACY, K3, Tracur, Gatak & Accuracy (avg.) - 96.97\% \\
\hline

\cite{ni2018malware} & SimHash, CNN, Bilinear Interpolation & 8*8, 8*16, 16*16, 16*32, 24*32, 28*32 &  10805 samples & Ramnit, Lollipop, Kelihos-ver3, Vundo, Simda, Tracur, Kelihos-ver1, Obfuscator.ACY, Gatak & Accuracy (Avg.) - 98.86\% \\
\hline

\cite{cui2018detection} & CNN, bats & Multiple representations depending on original file size & 9342 samples & 25 malware families as mentioned in the paper & Accuracy (Avg.) - 94.5\% \\
\hline

\cite{MD:Yue2017} & CNN and weighted softmax loss & vgg-verydeep-19 CNN model with 60 layers & 9342 samples & 25 malware families as gien in the paper & Accuracy-98.63\% \\
\hline

\cite{yan2018detecting} & CNN, LSTM, Truccated backpropagation Algorithm & 64*64 grayscale image & 21,736 samples & Ramnit, Lollipop, Kelihos-ver3, Vundo, Simda, Tracur, Kelihos-ver1, Obfuscator.ACY, Gatak & Accracy - 99.88\% \\
\hline

 \cite{su2018lightweight} & CNN & 64*64 grayscale image & 500 malware samples & Linux.Gafgyt.1, Linux.Gafgyt, Mirai, Trojan.Linux.Fgt, Tsunami, Hajime, LightAidra & Accuracy (2-class) - 94.0\% \newline Accuracy (3-class) - 81.8\% \\
 \hline
 
 \cite{le2018deep} & CNN, CNN-UniLSTM, CNN-BiLSTM & 10000 byte file size & 10,868 samples & Ramnit, Lollipop, Kelihos-ver3, Vundo, Simda, Tracur, Kelihos-ver1, Obfuscator.ACY, Gatak & Accuracy(CNN) - 95.8\% \newline Accuracy (CNN-UniLSTM) -  98.12\% \newline Accuracy(CNN-BiLSTM) - 98.20\% \\
 \hline
 
 \cite{kalash2018malware} & CNN & same as \cite{MD:Nataraj2011} & Malimg - 9,339 samples \newline Microsoft - 1868 samples & Malimg - 25 malware familes \newline Microsoft - 9 malware families & Accuracy (Malimg) - 98.52\% \newline Accuracy (Microsoft) - 99.97\% \\
 \hline
 
 \cite{cao2018efficient} & CNN & 2-D array with specified widths 28*28 / 56*56 & Vision Lab and Microsoft Datasets & 20 malware familes as mentioned in the paper & Accuracy - 95\% \\
 \hline


\end{tabular}
\end{table*}

%In \cite{MD:Wang2017}, they have proposed a malware traffic classification method using CNN by taking traffic data as images. The raw traffic data is directly input to the traffic classifier as a $28 \times28$ gray-scale image, and the classifier learn features automatically. The authors have claimed that the method has an average accuracy of 99.41\%. This method has advantages like protocol independent, early malware detection and high accuracy rate; however they haven't done parameter tuning, have ignored temporal features and the method cannot identify unknown malware traffic.

%\subsection{Mobile Malwares}
%Jiao et al. \cite{MD:Jiao2015} have proposed a method called ImageStruct to detect repackaged apps using similarity measurement.  In order to handle the large number of apps in the marketplaces, they have extracted distinguishing features from app images using pHash and compared the hash codes to detect the similar apps. When the similarity of two apps with different signatures exceeds a certain threshold, one of the apps was considered as repackaged.  In \cite{MD:Kywe2015}, they have proposed a text-based  and content-based image retrieval method to detect third-party applications on mobile market places. For each application, they have created a name index, description index, icon index and screenshot index. Text retrieval engines created name and description indexes, while icon and screenshot indexes were handled by image retrieval engine. For the image indexing, color correlogram algorithm was used. In the detection method, different intersection sets of the four retrieved sets were used and authors claimed that the result sets contain a total of 9.22\% of false positive.

%Long et al. \cite{MD:Long2014} have proposed a method to identify and visualize similarity between malware samples based on their embedded graphical assets. First, images were extracted from malware using wrestool and converted to 1024 dimensional vector using average hash. Then the vectors were stored using Fast Library for Approximate Nearest Neighbor (FLANN) index. Finally the top $n$ visually similar images were retrieved by the random tree method using $L2$ distances. The authors were claimed that the method has a recall of 83\% and precision of 85\%. Since the method uses average hashing and FLANN indexing, it is fast, however the performance is highly depending on the threshold values. 

%Malicious software detection based on a image classification method was proposed by Zhou et al. \cite{MD:Zhou2017}. The malware was visualized as a gray-scale image and all 512 GIST features were extracted by Gabor filter. Then extremely randomized trees method was used to classify the malware. To improve the system performance they have used the cross validation method, which requires more time and memory. This method has an accuracy of 96.2\%. 
%To reduce the run time and memory, Yajamanam et al. \cite{MD:Yajamanam2018} have evaluated the malware detection accuracy against the number of GIST features. They have concluded that a significant performance can be achieved by using only 60 GIST features. Then they have proposed a malware detection and classification method using 60 GIST features and k-NN classifier. In the classifier they have considered $k = 1$ and has achieved an accuracy of 93\%. However, this method is less efficient when there is large number of malware samples.

%A malware family classification method based on ensemble learning was proposed by Liu et al. \cite{MD:Liu2016}. The malware files were converted into a gray-scale image and compressed by the local mean method to a $512 \times 512$ image. To identify the malware families, ensemble learning based on bagging and K-means were used. This method was evaluated using twenty thousand malware samples from 20 malware families and has achieved 98.2\% accuracy. Even though this method avoids conflicts between classifiers using k-mean and bagging methods, it requires time to train the malware classifier.

%Choi et al. \cite{MD:Choi2017} have proposed a malware detection and classification method based on CNN. The malware was converted into $32 \times 32$ gray-scale image and input to a CNN. To make the model more robust, three convolution layers were used in the model. The evaluation was carried out using 2000 malware samples and the model has achieved an accuracy of 96\%. Kabanga et al. \cite{MD:Kabanga2018} have proposed a CNN model with cross entropy to detect malware families. First, the malware was converted into $128 \times 128$ gray-scale image and input to a CNN with three layers. The output layer has 25 neurons as they have considered 9458 malware samples from 25 malware families. Cross entropy loss function was used to optimize the output and authors have claimed that they achieved 98\% accuracy. 

\begin{table*}
\scriptsize
\centering
\caption{Traffic Anomaly Detection Approaches} \vspace{-3mm}
\begin{tabular}{|p{.8cm}|p{2cm}|p{3.5cm}|p{2.7cm}|p{2.2cm}|p{3.5cm}|}

 \hline
    \textbf{Ref}	& \textbf{Methods Used}	& \textbf{Advantages} & \textbf{Dataset (Normal/ Anomaly)} &\textbf{Comparison Vector}& \textbf{Performance Metrics}\\ \hline
    
    \hline
\multicolumn{5}{c}{\textbf{Image Representation Approaches}} \\ \hline
\hline

\cite{AD:Kim2005_netviewer1}\newline \cite{AD:Kim2005} &	DCT 	& Simple method that have considered only few features such as source/ destination address &	 3616/ 729	 & $4 \times 4$ DCT coefficients & \textbf{Source Address}-\newline Acc.- 92.3\%, FP- 0.3\%  \newline \textbf{Destination Address}-\newline Acc.- 87.2\%, FP- 0.75\% \\ \hline
 
\cite{AD:Kim2006} &	DCT and image pixels &	Have proposed a real time attack detection method	& 3563/ 782 & 1024 length vector and $4 \times 4$ DCT coefficients &	\textbf{Real-time analysis} \newline TP-92.8\%, FP-0.42\% \newline \textbf{Postmortem analysis} \newline TP-94.8\%, FP- 0.20\% \\ \hline

\cite{AD:Fontugne2008	} & Hough Transform & This method can be applied easily to any other traffic feature &	630/ 2000	& N/A & Acc.- 73.8\% \\ \hline

\cite{AD:Jeong2010} &	Hough Transform and CCL	& Attacks are detected by using a two tier architecture & N/A	 & N/A & N/A \\ \hline

\cite{AD:Tan2015} &	EMD	 & Detect attacks in a prompt manner &	\textbf{KDD cup 99:} \newline 97,260/ 3,892,550 \newline \textbf{ISCX 2012 IDS:} \newline 2,450,329/ 8720	& N/A & \textbf{KDD cup 99:} \newline Acc.-99.95\%, FP-1.93\% \newline \textbf{ISCX 2012 IDS:} \newline Acc.-90.12\%, FP-7.92\%  \\ \hline
  
\cite{AD:Li2017} &	CNN	& CNN uses the image form of data as input without feature selection & \textbf{NSL-KDD: } \newline \textbf{Test$^{+}$: }\newline 9711/12833 \newline  \textbf{Test$^{-21}$:} \newline 2152/9698 & $8\times 8$ input image to two CNNs (ResNet 50 and GoogLeNet) &  \textbf{ResNet 50:} \newline \textbf{Test$^+$:} Acc.- 79.14\% \newline \textbf{Test$^{-21}$:} Acc.- 81.57\% \newline \textbf{GoogleNet:}\newline \textbf{Test$^+$:} Acc.- 77.04\% \newline \textbf{Test$^{-21}$:} Acc.- 81.84\% \\ \hline
  
 \cite{AD:Zou2018} &	 GLCM texture features &	A spatial and temporal analysis of network resources were carried out, and the method has reduced the complexity by using textural features &	100 CPS device traffic	& Size of the image is eual to number of CPS devices in the system& Acc. - 99\% \\ \hline

\cite{AD:Martin2017} &	CNN and RNN	& The system is more robust with high detection rate &	RedIRIS-  266,160 network flows	& 6 features and 5-15 packets & Acc. 96\% \\ \hline

\end{tabular}
\end{table*}

    \item \textbf{Malware Families:} We realized that most of the abovementioned techniques are tested/validated on a same set of malware families. The commonly used malware families are 
    \texttt{Ramnit, Lollipop, Kelihos-ver3, Vundo, Simda, Tracur, Kelihos-ver1, Obfuscator.ACY, and Ghatak} provided by Microsoft Challenge dataset. In addition, we realized that these malware families are mostly used by CNN-based techniques. We also found another set of common malware families used by researchers from Malimg Datasets. These are \texttt{Allaple.L, Allaple.A, Yuner.A, lolyda.AA 1, lolyda.AA 2, lolyda.AA 3, C2Lop.P, C2Lop.gen!G, Instantaccess, Swizzor.gen!I, Swizzor.gen!E, VB.AT, Fakerean, Alueron.gen!J, Malex.gen!J, Lolyda.AT, Adialer.C, Wintrim.BX, Dialplatform.B, Dontovo.A, Obfuscator.AD, Agent.FYI, Autorun.K, Rbot!gen, Skintrim.N} respectively. There are only very few techniques that are regressively tested on a large set of malware families. For-example, we found only Han et al. \cite{han2015malware} that has performed their experiments on 50 different malware families.
    
    \item \textbf{Datasets:} Most of the researchers have utilized Microsoft Malware Classification Challenge (BIG 2015) as the validation dataset for their techniques. This dataset has 0.5 terabyte size, consisting of disassembly and bytecode of more than 20K malware samples. Another malware datasets which is most often used for detection is the Malimg dataset. This malware dataset contains 9,339 malware samples from 25 different malware families. We also found a technique proposed by \cite{trinius2009visual}  that has set-up honeypots in a controlled network environment for the real-time malware detection.
    
    To avoid phishing attacks, a general yet more reliable approach is to detect a phishing attempt before users click a malicious url, thus preventing them to be victimized. In this regard, there are two automated phishing attack detection methods: i) blacklist based methods and ii) text similarity-based methods. Blacklist-based methods attempt to keep a list of domain names or exact URLs to known phishing websites and alert users if they are trying to visit those links. However, currently phishing websites are highly dynamic and average lifetime of a phishing webpage is only few hours \cite{zdnet}. Text similarity-based methods delves into semantics of the textual content, be it an email, web page, or a mobile app and try to decide whether it is a phishing attempt or not.  For example, such solutions may focus on the similarity of the URLS (e.g. \texttt{www.google.com} vs. \texttt{www.goole.com}). Also, these methods will assess the text content of the web page/email or app description and use text mining methods to predict whether the links included in the body of text is phishing or not. However, this method suffers from code obfuscation problem as similarity cannot be checked if the content is obfuscated. In addition, latest phishing attempts prompt users with highly visually similar websites to popular websites or embed forged visual content such as logos to present misleading information. Such attempts will not be detected by above methods and it is necessary to develop phishing detection tools that can accommodate visual similarity between web pages, software GUIs, or mobile apps. Therefore, computer vision-based techniques have been proposed to detect traditional as well as more sophisticated phishing attacks. In Section \ref{sec:PWA}, we investigated such computer-vision based techniques, in an attempt to highlight the significance of this computer vision in detecting phishing attacks.
    
    In an attempt to detect and classify malware types, most organizations rely on two traditional approaches, static code analysis (signature-based) or dynamic code analysis (behavior-based). Static code analysis protect systems and networks from known threats and attacks. A static code is a short sequence of bytes unique to each known malware, which allows newly encountered malicious files to be correctly flagged malicious with a small error rate. This type of detection method is less responsive to a new malware and also suffers from malware code obfuscation problem. Moreover, it may even allow variants of same malware to bypass the detection and stay undetected for a long time. On the other hand, methods based on dynamic code analysis (behaviour-based), can detect malware based on the activities exhibited by malware during runtime. This type of detection method does not suffer from the limitations found in signature-based techniques, however, it gives high false positive rate where a benign program is falsely classified as a malicious program. Additionally, dynamic code methods are computationally expensive and require a lot of resources for proper execution. To alleviate the problems of above two detection approaches such as code obfuscation, expensive computations, techniques from computer vision have been recently utilized. Computer vision techniques have a capability of detecting malware even if the code is obfuscated and are less computationally expensive than dynamic analysis methods. Computer vision also speedups detection process by providing a summarized picture of possible attack through visual representation. All in all, the use of computer vision techniques to detect malware offer several benefits that need to be investigated and therefore, in Section \ref{sec:MDA}, we attempt to provide detailed analysis of malware detection approaches.
    
    In order to detect the abnormalities and attacks in network traffic, the two major approaches have been developed i.e. signature-based approach and anomaly-based approach. In the signature-based approach, anomaly is detected based on predefined signatures, which are built on the basis of the characteristics and features of previously known attacks. The limitation of this approach is that it requires the signature to be known beforehand, and it is not capable to detect new anomalies. In the second approach, the detection methods are based on certain underlying models, which are labeled based on traffic normal behavior. These methods detect and characterize anomalous patterns in the traffic based on deviation from the underlying labeled models. Once the traffic is characterized anomalous, then the corresponding data is investigated more closely to identify the root cause of the anomaly. This approach does not require any prior knowledge about the anomalies, and it is capable of discovering new anomalies. However, the problem with this approach is defining the rule set i.e. efficiency of a detection system depends on how well rule set is implemented and tested on all protocols. Moreover, a variety of custom protocols that are used by different vendors makes the rule defining process difficult. In addition, this approach also suffers from false positive rate e.g. an activity such as directory traversal on a targeted vulnerable server, which complies with network protocol, easily goes unnoticed as it does not trigger any alert. Thus, there is a need of an anomaly detection system that not only overcomes the problems of above two approaches but also offers faster diagnosis, lower complexity, and high precision. In this regard, researchers proposed traffic anomaly detection systems based on computer vision techniques as there are few commonalities shared between network anomaly detection and computer vision tasks, such as image retrieval and object shape recognition. For instance, normal traffic to DoS attack detection can be equivalent to queries to image retrieval tasks or object shape recognition tasks. DoS attack can be interpreted as the images or the object shapes that do not match the queries. In Section \ref{sec:ADA}, we analyzed few traffic anomaly detection methods, that are based on computer vision.
